CoCo: Coherence-Enhanced Machine-Generated Text Detection Under Data Limitation With Contrastive Learning

Machine-Generated Text (MGT) detection, a task that discriminates MGT from Human-Written Text (HWT), plays a crucial role in preventing misuse of text generative models, which excel in mimicking human writing style recently. Latest proposed detectors usually take coarse text sequences as input and fine-tune pretrained models with standard cross-entropy loss. However, these methods fail to consider the linguistic structure of texts. Moreover, they lack the ability to handle the low-resource problem which could often happen in practice considering the enormous amount of textual data online. In this paper, we present a coherence-based contrastive learning model named CoCo to detect the possible MGT under low-resource scenario. To exploit the linguistic feature, we encode coherence information in form of graph into text representation. To tackle the challenges of low data resource, we employ a contrastive learning framework and propose an improved contrastive loss for preventing performance degradation brought by simple samples. The experiment results on two public datasets and two self-constructed datasets prove our approach outperforms the state-of-art methods significantly. Also, we surprisingly find that MGTs originated from up-to-date language models could be easier to detect than these from previous models, in our experiments. And we propose some preliminary explanations for this counter-intuitive phenomena. All the codes and datasets are open-sourced.

==> Body/Exp_Discussion.tex <==
\section{Experiments \& Discussion}




% This section discusses a set of experiments to evaluate the utility and sensibility of \sysname, including methods comparison, ablation study, and case study. Then we examine the effect of hyper-parameters. Moreover, we propose a further discussion around three in-depth questions for \sysname.


\subsection{Performance Comparison}

As shown in Table \ref{table:2}, our method surpasses state-of-the-art methods in MGT detection task by at least \textbf{0.31} and \textbf{0.96} in terms of accuracy and F1-score on limited GROVER dataset. And it outstrips at least \textbf{0.16} accuracy and \textbf{0.13} F1-score on limited GPT-2 dataset.
On full dataset, \sysname outperforms other models by at least \textbf{0.44} and \textbf{0.63} in metrics of accuracy and F1-score on GROVER. \sysname also towers above at least \textbf{0.49} accuracy and \textbf{0.62} F1-score on GPT-2 dataset.

Moreover, our model also excels the test result reported by GROVER and FAST. 
The accuracy score of GROVER-Base with about the same size of \sysname is 80.0 on its dataset \citep{RowanZellers2019DefendingAN}. 
And FAST reports its accuracy on GROVER is 84.90 and on GPT-2 is 93.10 \citep{WanjunZhong2020NeuralDD}. 
Our \sysname outperforms both of them.

It indicates that \sysname has significant power of mining distinguishable features and suits for both low-resource and high-resource environment.
Moreover, it should be noticed that \sysname gets less affected by randomness, which illustrates that the coherence graph we construct is a robust feature that helps stabilize the model performance.
Additionally, we find that the randomness intensely impacts DualCL, and the model is very prone to failure, leading to a large standard deviation in \tabref{table:2}. 
It is because DualCL is mainly focused on evaluating short texts which contains only few words (around 10 words) and is not suitable for long-term evaluation. 
% Also, the performance of DualCL is highly influenced by the embedding of labels' names, which is not in the same representation spatial of long documents.


% In Table \ref{table:2}, Roberta performs the best among the Transformers based fine-tuning methods and can bear low-resource limitations. Hence, the models of Contrastive Learning based methods and \sysname are built based on Roberta. The SCL method shows enhanced performance, especially on the limited dataset. Furthermore, FAST outperforms the formal fine-tuning methods, which proves that graph-based structure information can improve detection. Overall, ignited by all the previous works, our model, \sysname and its derivatives, significantly outperforms all the datasets, incredibly robust under the dataset size limitation. \TODO{metion the acc num}  


\subsection{Ablation Study}

To illustrate the necessity of every part of our \sysname and their enhancement to the model performance, we carry out five groups of ablation experiments as follows. By ablation and derivation, trials embody \sysname's structure reliability and extension potentials. \tabref{table:ab} shows the results of the ablation study. A detailed explanation of our ablation settings is as follows. The dataset here is 10\% GROVER.



\begin{table}[!h]
\centering
\renewcommand\arraystretch{1.2}
\begin{tabular}{lcc}
\bottomrule
\textbf{Model}                           & \textbf{ACC}                 & \textbf{F1}                  \\ \bottomrule
% {\color[HTML]{656565} fine-tune RoBERTa} & \cellcolor[HTML]{69c0f3}{77.30}                        & \cellcolor[HTML]{77d0ff}{63.70} \\ 
w/o Graph \& CL                          & \cellcolor[HTML]{77d0ff}76.97                          & \cellcolor[HTML]{64baea}{64.28}                        \\ 
w/ Sent. Graph w/o CL                     & \cellcolor[HTML]{69c0f3}{77.33}                        & \cellcolor[HTML]{6dc5fa}{63.79}                        \\ 
% {\color[HTML]{656565} SCL}               & \cellcolor[HTML]{47a3d7}{77.77}                        & \cellcolor[HTML]{5aaee1}{64.47} \\ 
w/ Graph w/o CL \& LSTM                   & \cellcolor[HTML]{47a3d7}{77.77}                        & \cellcolor[HTML]{47a3d7}{64.63}                        \\ 
w/ Graph w/o CL                           & \cellcolor[HTML]{3d97cd}{77.87}                        & \cellcolor[HTML]{3d97cd}{64.71}                        \\ 
w/ Graph \& SCL                                    & \cellcolor[HTML]{338bc3}{78.27}                        & \cellcolor[HTML]{338bc3}{66.09}                        \\ \hline
\textbf{\sysname}         & \cellcolor[HTML]{2980b9}{78.43}                            & \cellcolor[HTML]{2980b9}{66.84}                           \\ \bottomrule
\end{tabular}
\caption{Results of Ablation Study}
\label{table:ab}
\end{table}



\fakeparagraph{w/o Graph \& CL} removes graph information and encodes only by RoBERTa parts. Moreover, the model removes contrastive learning and uses CE loss.

\fakeparagraph{w/ Sent. Graph w/o CL} treats sentences as nodes instead of entities and removes contrastive learning and uses CE loss.

\fakeparagraph{w/ Graph w/o CL \& LSTM} removes contrastive loss and replace LSTM in encoder with average pooling operation.

\fakeparagraph{w/ Graph w/o CL} uses LSTM for document-level aggregation and the rest is the same as w/ Graph w/o CL \& LSTM.

\fakeparagraph{w Graph \& SCL} replaces the improved contrastive loss with traditional supervised contrastive loss.

As shown in \tabref{table:ab}, we can see that \sysname outperforms baseline models even after ablation. Though the performance of ablated models slightly drops compared to the completed \sysname. This result proves the feasibility and sensibility of our design of \sysname architecture and shows its potential to extend.

\subsection{Effect of Hyper-Parameters}

\subsubsection{Contrastive Learning Parameters}

We evaluate the influence of contrastive learning hyper-parameters $\alpha$ and $\tau$ with experiment on different combination of them. 
The result is shown in figure \ref{fig:modelpa}.
Considering the discovering that smaller $\tau$ leads to better hard negative mining ability \ref{wang2021understanding}, we select $\alpha$ from ${0.2,0.4,0.6,0.8}$ and $\tau$ from ${0.1,0.2}$.
We find that the extreme $\alpha$ value causes the performance degradation and the best hyper-parameter combination is $\alpha, \tau=0.6, 0.2$.
Our analysis is that large $\alpha$ forces the model to concentrate on the instance-level contrast and small $\alpha$ lets class separation objective take control.
Both will reduce the generalization performance of the detector on test set.

% For contrastive learning hyper-parameters, a grid search strategy is implemented to choose an appropriate combination for $\alpha$ from $ 0.1$ to $0.9 $ in Eq.\ref{tot} and $\tau \in \left \{ 0.1, 0.2, 0.3 \right \} $ in Eq.\ref{scl}. $\alpha$ adjusts the relative balance between instance compactness and class separability in the total loss, and $\tau$ is the temperature hyperperameter for evaluating similarity in our supervised contrastive loss.

% \begin{table*}[]
% \renewcommand\arraystretch{1.5}
% \centering
% \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
% \bottomrule

% \end{table*}


% \begin{table*}[]
% \renewcommand\arraystretch{1.5}
% \centering
% \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
% \bottomrule
%              & \textbf{0.1}                                            & \textbf{0.2}                                            & \textbf{0.3}                                            & \textbf{0.4}                                            & \textbf{0.5}                                            & \textbf{0.6}                                                     & \textbf{0.7}                                            & \textbf{0.8}                                            & \textbf{0.9}                                            \\ \bottomrule
% \textbf{0.1} & \begin{tabular}[c]{@{}c@{}}0.7740\\ 0.7745\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7607\\ 0.7673\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7527\\ 0.7413\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7613\\ 0.7639\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7587\\ 0.7567\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7783\\ 0.7803\end{tabular}          & \begin{tabular}[c]{@{}c@{}}0.7703\\ 0.7613\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7587\\ 0.7644\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7510\\ 0.7623\end{tabular} \\ \hline
% \textbf{0.2} & \begin{tabular}[c]{@{}c@{}}0.7743\\ 0.7722\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7704\\ 0.7700\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7611\\ 0.7623\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7560\\ 0.7553\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7630\\ 0.7654\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}0.7857\\ 0.7825\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.7583\\ 0.7577\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7317\\ 0.7251\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7633\\ 0.7727\end{tabular} \\ \hline
% \textbf{0.3} & \begin{tabular}[c]{@{}c@{}}0.7553\\ 0.7608\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7453\\ 0.7479\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7547\\ 0.7551\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7450\\ 0.7432\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7610\\ 0.7650\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7733\\ 0.7774\end{tabular}          & \begin{tabular}[c]{@{}c@{}}0.7543\\ 0.7623\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7473\\ 0.7469\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.7600\\ 0.7608\end{tabular} \\ \bottomrule
% \end{tabular}
% \caption{Grid Search for $\alpha$ and $\tau$.  The horizontal side of the table is the value of $\alpha$ and the vertical side is $\tau$. The first row of each cell is the accuracy at evaluation, and the second row is the accuracy at test.}
% \label{table:grid2}
% \end{table*}

% In figure \ref{fig:modelpa}, we observe that our model performs best overwhelmingly with the hyper-parameter combination $\alpha=0.6$ and $\tau=0.2$. The two parameters do not perform better with larger or smaller values. \yichen{Need to be discuss} For $\alpha$, the moderate value reflects the complementarity between $\mathcal{L}_{\text{ICL}}$ and $\mathcal{L}_{\text{CE}}$. And $\tau$ shows the suitable correspondence between text similarity distribution and loss function.

\begin{figure}[!h]
  % \hspace{-7em}
  \centering
  \includegraphics[width=\linewidth]{Figure/para.png}
  \caption{Effect of parameter $\alpha$ and $\tau$ on model performance}
  \label{fig:modelpa}
  \vspace{-0.5cm}
\end{figure}

\subsubsection{Graph Parameters}

We further investigate the effect of max node number and max sentence number on model performance.
The result is shown in Fig \ref{fig:graphpa}.
We select max node number from $\{ 60,90,120,150 \}$ and max sentence number from $\{ 30,45,60,75 \}$.
The detector performs best when max node number is 90 and max sentence number is 45.
The experiment results prove that the large node and sentence number are not necessary for the improvement of detection accuracy.
We infer that even though setting large node and sentence number includes more entity information, excessive nodes bring noise to the model and impair the distinguishability of coherence feature.

\begin{figure}[!h]
  % \hspace{-7em}
  \centering
  \includegraphics[width=1.1\linewidth]{Figure/Abl.png}
  \caption{Performance of Model with Different Graph Parameters}
  \label{fig:graphpa}
  \vspace{-0.5cm}
\end{figure}

\subsection{Analysis and Discussion}

\subsubsection{How does the coherence graph help detection?}

We apply static geometric features analysis to coherence graph we construct to evaluate the distinguishable difference between HWTs and MGTs with explanation. 
% Static geometric features analysis is commonly used in the domain of computer networks. 
% We propose that a similar analysis can quantify the complex interaction in the long-term text.
In the following discussion, we take the dataset of GROVER into the analysis.
Some basic metrics of data and the corresponding graph are shown in Table \ref{basic}. 

\begin{table}[!ht]
\centering
\begin{tabular}{l|l|l}
\hline
\textbf{Metric}      & \textbf{HWT} & \textbf{MGT} \\ \hline
Sample Num.          & 4994         & 4991         \\ \hline
Avg. Num. of Token   & 463.2        & 456.0        \\ \hline
Avg. Num. of  Vertex & 43.60        & 32.37        \\ \hline
Avg. Num. of Edge    & 107.4        & 65.44        \\ \hline
\end{tabular}
\caption{Basic Metrics of Texts and Corresponding Graphs}
\label{basic}
\end{table}

% Though HWTs and MGTs have approximately the same number of tokens in every text, coherence graph for HWTs has larger scale than MGTs’ with \textbf{34.7\%} more vertexes and \textbf{64.1\%} more edges, which shows that HWTs have more complex semantic relation structures than MGTs.

\fakeparagraph{Degree Distribution}
%The degree of a vertex is the number of edges that are incident to the vertex, and degree distribution is the probability distribution of degrees over the whole graph.
of coherence graph semantically measures the co-occurrence and TF-IDF feature of keywords, showing global coherence because high-degree nodes devote to the main topic and low-degree nodes are the extension.
%As shown in \tabref{deg}, 
The degree of the graph representation of HWTs is \textbf{2.980}, which is \textbf{15.0\%} larger than MGTs (2.591),
%which shows disparities of MGTs to form coherent interaction between sentences. \figref{fdeg} measures the distribution of each graph's average nodes' degree, showing that 
and the distribution of HWTs has a longer tail than MGTs.
% \begin{figure}[!ht]
% \begin{minipage}{.4\linewidth}
%     \centering
%     \renewcommand\arraystretch{1.3}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|c}
%     \hline
%     \textbf{Metric}        & \textbf{Avg. Degree} \\ \hline
%     \textbf{HWT}           & 2.980 \\ \hline
%     \textbf{MGT}           & 2.591 \\ \hline
%     \end{tabular}
%     }
%     \captionof{table}{Avg of Degree (Whole Dataset) }
%     \label{deg}
% \end{minipage}
% \hfill
% \begin{minipage}{.47\linewidth}
% \centering
% \includegraphics[width=1.1\linewidth]{Figure/AvgDegofGraph.png}
% \caption{Distribution of Avg. Degree of Graphs}
% \label{fdeg}
% \end{minipage}
% \end{figure}
Furthermore, we prove that degree distribution can robustly detect MGTs and HWTs when impacted by style and genre differences in \ref{app:static}.

% \begin{figure}
%     \centering
% \includegraphics[width=1\linewidth]{Figure/degtot.png}
%     \caption{Distribution of Degree with different provenance}
%     \label{fig:dpro}
% \end{figure}

%Furthermore, we analyze the distinguishability of degree features when impacted by other factors. One most considerable influences is the style and genre of different provenance. We chose around 60 articles from The Sun\footnote {https://www.thesun.co.uk/} and Boston\footnote {https://www.boston.com/}. Then we use GROVER to mimic their style to generate similar topic news. \figref{fig:dpro} shows the degree distribution of HWTs and MGTs of both provenances. 



% We use Jensen–Shannon divergence to evaluate the similarity of the degree distribution. 
% % The minor JS divergence is, the more similar the two distributions are. 
% The JS-divergence of MGTs mimicking TheSun and Boston is \textbf{0.029}, while the JS-divergence of MGTs and HWTs in Boston is \textbf{0.050}, in TheSun is \textbf{0.061}. The apparent gap shows that degree distribution can robustly detect MGTs and HWTs when impacted by provenance differences.

% \fakeparagraph{Aggregation}
% %is a shared metric for complex networks and linguistics, 
% depicts how closely the whole is organized around its core. We propose two metrics to evaluate the aggregation of graph-based text representation in our coherence model, the size of the largest connected subgraph and the clustering coefficient in \ref{app:static}. their distribution are distinguishable in \figref{lcs} and \figref{fcc}.

% % In our representation, not all sentences have entities related to others. Hence the graph is an unconnected one. The average number of nodes in subgraphs of MGTs is \textbf{4.49} and of HWTs is \textbf{4.84}. We propose that the size of the largest connected subgraph shows the contents which are closely organized around the topic. Moreover, the size of graphs may be an unfair factor, so we use the portion of nodes in the largest connected subgraph to reflect its size. The average portion in HWTs is \textbf{0.6725} and in MGTs is \textbf{0.6458}. \figref{lcs} shows the distribution of the portion of graphs, and HWTs distribute more high-portion ones than MGTs.

% \begin{figure}[!ht]
% \begin{minipage}{.47\linewidth}
% \centering
% \includegraphics[width=\linewidth]{Figure/lcs.png}
% \caption{Portion of the Largest Connected Subgraph}
% \label{lcs}
% \end{minipage}
% \hfill
% \begin{minipage}{.47\linewidth}
% \centering
% \includegraphics[width=\linewidth]{Figure/cc.png}
% \caption{Distribution of Clustering Coefficient}
% \label{fcc}
% \end{minipage}
% \end{figure}

%The clustering coefficient represents how nodes tend to cluster. For the entities of texts, clustering evaluates how the author narrates around the central theme. The larger the clustering coefficient is, the tighter the semantic structure is. The average cluster coefficient of the graphs of HWTs is \textbf{0.2213} and of MGTs is \textbf{0.1983}, HWTs is \textbf{11.6\%} better than MGTs. \figref{fcc} shows the distribution.

\fakeparagraph{Core \& Degeneracy}
The degeneracy of a graph is a measure of how sparse it is, and the $k$-core is the subgraph corresponding to its significance in the graph. We propose that,  in our graph representation,  the degeneracy process of graphs equals summarizing texts semantically. The maximum of core-number shows the complexity of hierarchical structure in texts. Furthermore, the distribution of the core-number reflects the overall sparse and is a graph-perspective N-gram module. Based on experiments, the average core-number of HWTs is \textbf{5.772} while MGTs with \textbf{4.458}. HWTs are \textbf{29.5\%} ahead. \figref{kc} is the distribution of the core-number.

\begin{figure}[!ht]
\begin{minipage}{.47\linewidth}
\centering
\includegraphics[width=\linewidth]{Figure/kc.png}
\caption{Core-number of Nodes in Graphs}
\label{kc}
\end{minipage}
\hfill
\begin{minipage}{.47\linewidth}
\centering
\includegraphics[width=\linewidth]{Figure/en.png}
\caption{Structure Entropy of Graphs}
\label{fen}
\end{minipage}
\end{figure}

\fakeparagraph{Entropy} 
%Entropy is a scientific concept to measure a state of disorder, randomness, or uncertainty. The well-known Shannon entropy is the core of the information theory, measuring the self-information content. For the graph data, network structure entropy defined as the following can examine the information amount of the graph structure.
We propose global coherence equals refining more information inside the semantic structure of the whole text, which matches to structure entropy of our graph representation. From our experiments, the structure entropy of HWTs (2.263) is \textbf{6.80\%} larger than MGTs (2.119), which means HWTs obtain more structured information because their semantic information is globally organized. We show the distribution in \figref{fen}.

\begin{equation}
    E=-\sum_{i=1}^N I_i \cdot \ln I_i = -\sum_{i=1}^N \frac{k_i}{\sum_{j=1}^N k_j} \cdot \ln( \frac{k_i}{\sum_{j=1}^N k_j})
\end{equation}





% \yichen{@zhaohan, need you to polish this part! }
% For our graph representation, two parameters impact the performance the most, the number of nodes and the number of sentences of aggregation. To improve our performance, we conduct a grid search for them, as the results are shown in the \figref{fig:graphpa}. The test is based on the full dataset of GROVER.
% Based on the result, we found that increasing the node number and sentence representation number only sometimes enhances performance. Since the larger the constructed graph or the aggregated graph is, the density of the representation will decrease and negatively affect the performance. Finally, with the limitation of the token number 512, we set the node number as 90 and the sentence number as 45.

% \subsubsection{Generalization Capability}

% \yichen{todo}

% \subsubsection{Question three.}

% \yichen{my opinion: talk about imbalanced situation}

% \subsection{Shortcomings}

% \yichen{todo}

==> Body/ProblemDefinition.tex <==
\section{Problem Formulation}

This work aims to distinguish MGT from HWT with data limitation, which often happens in real scenarios.
The problem could be explained as a binary low-resource classification problem.
Given a susceptible document $d$ with $n$ sentences, the model is required to distinguish whether $d$ is MGT or HWT in a supervised fashion with auxiliary information from coherence graph $G_c = \{ \mathcal{V}, \mathcal{E} \}$ extracted from $d$.
Therefore, this detection problem could be defined simply as follows.
% represent coherence by graph $G_c = \{ \mathcal{V}, \mathcal{E} \}$.
% Use a supervised method to distinguish whether the text is MGT or HWT.
% Therefore, this detection problem could be defined simply as follows.

%We study the problem of deepfake text detection.
% This work aims to distinguish MGT from HWT with data limitation which often happens in real scenarios.
% The problem could be explained as a binary low-resource classification problem.
% Given a susceptible document $d$ with $n$ sentences, coherence model based on graph representation $G_c = \{ \mathcal{V}, \mathcal{E} \}$  is constructed to indicate the interactions among the sentences.\yichen{needed?}
% After encoding the coherence graph and text sequence into latent representations, a supervised contrastive learning model is designed to distinguish the text.
% Therefore, this detection problem could be defined simply as following.
%We conduct our experiment on two datasets following (\citealp{zhong2020neural}), which are news-style dataset with fake text generated by GROVER(\citealp{zellers2019defending}) and large-scale webtext-style dataset with fake text generated by GPT-2(\citealp{radford2019language}) respectively and we manipulate the training set to be small and imbalanced to simulate real scenario.

\noindent \textbf{Input:} 
A  document set $S_d=\{d_1, d_2, \ldots, d_k\}$.

\noindent \textbf{Output:} 
With the given dataset, the model is required to make the judgement about which ones are human-written and which ones are machine-generated, \ie  a set of label $S_L$ in return.




